Between the AI and Me: Analysing Listeners' Perspectives on AI- and Human-Composed Progressive Metal Music

Generative AI models have recently blossomed, significantly impacting artistic and musical traditions. Research investigating how humans interact with and deem these models is therefore crucial. Through a listening and reflection study, we explore participants' perspectives on AI- vs human-generated progressive metal, in symbolic format, using rock music as a control group. AI-generated examples were produced by ProgGP, a Transformer-based model. We propose a mixed methods approach to assess the effects of generation type (human vs. AI), genre (progressive metal vs. rock), and curation process (random vs. cherry-picked). This combines quantitative feedback on genre congruence, preference, creativity, consistency, playability, humanness, and repeatability, and qualitative feedback to provide insights into listeners' experiences. A total of 32 progressive metal fans completed the study. Our findings validate the use of fine-tuning to achieve genre-specific specialization in AI music generation, as listeners could distinguish between AI-generated rock and progressive metal. Despite some AI-generated excerpts receiving similar ratings to human music, listeners exhibited a preference for human compositions. Thematic analysis identified key features for genre and AI vs. human distinctions. Finally, we consider the ethical implications of our work in promoting musical data diversity within MIR research by focusing on an under-explored genre.

==> Sections/ethical-statement.tex <==
\section{Ethical Statement}


==> Sections/results_OLD.tex <==
\section{Results}

\subsection{Listening Test}
We present violin plots visualizing the distribution of answers to questions Q1 to Q8 for each stimuli group  (progcp, progrand, proghum, rockcp, rockrand, rockhum). Additionally, we conducted statistical analyses to investigate the effects of the creation method on dependent variables. These analyses employed a Type I error rate ($\alpha$) of 0.05.
Due to the fact that the assumptions for normality are not met in the data samples, together with the characteristics of the test in which each participant rated stimuli from every group, we report results of a Friedman test, supported by a post-hoc pairwise Wilcoxon test, Bonferroni-adjusted $\alpha$ level of $.0033$ ($.05/15$). These findings are summarized in Tables \ref{tab:ft} to \ref{tab:q8wilcoxon} in the Appendix A section of this thesis.



\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_prog_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q1, ``This composition features the qualities of the progressive metal genre''. Violin plots combine aspects of box plots and kernel density plots, providing an estimation of the probability density function of the data.}
    \label{fig:isprog}
\end{figure}

From the plots in Figure \ref{fig:isprog}, we can observe an overall agreement that the groups concerned with the generation of compositions in the style of progressive metal (\textbf{progcp}, \textbf{progrand}, \textbf{proghum}) were deemed capable of creating content in said genre, by comparing it against the Rock generation groups (\textbf{rockcp}, \textbf{rockrand}, \textbf{rockhum}). The statistical results from the Friedman test showed a highly significant effect of the type of generation in the participants responses amongst groups, towards the question of whether or not the compositions feature qualities of the progressive metal genre ($\chi^2(5)=136.90$, $p<.001$). 

The post-hoc pairwise Wilcoxon test (presented in Table \ref{tab:q1wilcoxon} of Appendix A) demonstrated highly significant differences in ratings between groups, with the exception of the pairs \textbf{progcp-proghum}, \textbf{progcp-progrand} and \textbf{rockcp-rockrand}. This is particularly relevant when framed within the median scores obtained for \textbf{progcp} and \textbf{proghum}, as it suggests that the cherry-picked examples from ProgGP could be considered as having progressive metal features of similar quality of those of the human-generated group. Furthermore, the randomly selected examples from ProgGP (\textbf{progrand}) obtained a median score similar to \textbf{progcp}, which indicates that a random sampling of the ProgGP's output seems to have enough features that resemble the style of progressive metal. Similar conclusions can be said about the \textbf{rockcp-rockrand} pair, regarding the lack of significant statistical differences of between these groups for this particular question.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_rock_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q2, ``This composition features the qualities of the Rock genre''.}
    \label{fig:isRock}
\end{figure}

Concerning the question of a composition featuring qualities of the Rock genre, the plot in Figure \ref{fig:isRock} displays a violin plot for each of the groups. As hypothesized, the Rock generation groups seem to obtaining much higher ratings than the progressive metal ones. We report the results of the Friedman test, showing a highly significant effect of the type of generation in the participants responses towards the question of whether or not the compositions feature qualities of the Rock genre ($\chi^2(5)=110.09$, $p<.001$).

The post-hoc pairwise Wilcoxon test (presented in Table \ref{tab:q2wilcoxon} of Appendix A) showed highly significant differences in ratings between groups, with the exception of the pairs concerning the progressive metal group (combinations \textbf{progcp}, \textbf{progrand}, \textbf{proghum}) and \textbf{rockcp-rockrand}. These results suggest similar conclusions as those hypothesized for Q1, namely that a random sampling of the Rock generating model from Chapter \ref{ch5:GTR-CTRL} provides examples that have a similar level in terms of featuring qualities of the Rock genre as the cherry-picked examples. However, differently from the results in Q1, both rockcp and rockhum showed highly significant differences in ratings when compared to the human-generated Rock examples, suggesting that perhaps ProgGP is more capable of reproducing progressive metal examples that are deemed closer to human quality, than the model from genre-CTRL is of doing the same for the genre of Rock. This might be justified by the fact that the model in genre-CTRL was capable of generating compositions in other styles besides Rock (i.e. punk, Metal, classical and folk), thus making it theoretically more flexible and less constrained to the Rock genre, whereas ProgGP was fine-tuned on examples from the progressive metal genre exclusively.

Results for Q3 (``I like this composition'') can be seen in Figure \ref{fig:islikeable}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_likeable_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q3, ``I like this composition''.}
    \label{fig:islikeable}
\end{figure}

Similarly, statistical results from the Friedman test showed a highly significant effect of the type of generation in the answers towards the question of whether or not they like the auditory examples ($\chi^2(5)=77.56$, $p<.001$). 

As per the results from the pairwise Wilcoxon test (presented in Table \ref{tab:q3wilcoxon} of Appendix A), we highlight that within the Rock genre groups, there were no significant differences between the distributions of the answers for the AI-generated and the human-generated groups, although participants seem to overall prefer the human-created examples. Futhermore, the differences between the \textbf{progrand} and \textbf{proghum} groups obtained the highest statistical significance. 

For the results concerning Q4, displayed in Figure \ref{fig:iscreative}, we report a highly significant effect of the type of generation in the answers towards the question of whether or not participants deem these auditory examples as creative ($\chi^2(5)=88.54$, $p<.001$), as per the findings in the Friedman test. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_creative_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q4, ``This composition is creative''.}
    \label{fig:iscreative}
\end{figure}

From the results in pairwise Wilcoxon test (presented in Table \ref{tab:q4wilcoxon} of Appendix A) we observe that there was no statistical differences between the groups of \textbf{progcp} and \textbf{proghum}, suggesting that the cherry-picked examples from ProgGP express a level of creativity similar to those that were human-generated. In this regard, the opposite can be said about the comparison between \textbf{progrand} and \textbf{proghum}, with a highly significant difference between these two groups. Concerning the groups for the Rock genre, both comparisons between the AI-generated and human-generated groups showed no statistically significant differences in the distributions of the ratings, despite an overall higher median score for the \textbf{rockhum} group.

In Figure \ref{fig:isconsistent} and Figure \ref{fig:isplayable} we display plots concerning the answers to Q5 and Q6, assessing respectively the notions of consistency and playability.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_consistent_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q5, ``This composition is consistent''.}
    \label{fig:isconsistent}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_playable_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q6, ``This composition is playable''.}
    \label{fig:isplayable}
\end{figure}

For these questions we report a significant statistical differences between the effects of the type of generation groups for Q5 ($\chi^2(5)=42.50$, $p<.001$) and Q6 ($\chi^2(5)=55.47$, $p<.001$). However, as is observable from the plots in the corresponding figures, all the groups scored highly in both questions. Furthermore, results from the pairwise Wilcoxon test (presented in Table \ref{tab:q5wilcoxon} and Table \ref{tab:q6wilcoxon} of Appendix A) showed no significant statistical differences between groups.



Concerning Q7, the question of whether or not participants deemed the examples as generated using AI, often referred to as Musical Turing Test, we display the results in Figure \ref{fig:isAI}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_ai_nofam_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q7, ``This composition was generated using AI''. Entries for which participants declared familiarity with the stimuli were removed.}
    \label{fig:isAI}
\end{figure}

Due to the relevance of knowing a certain stimuli towards the question of whether or not participants thought it was generated using AI, we excluded from this analysis the entries for which participants stated that they were familiar with the auditory examples, discarding 345 responses (out of 1,920).
The Friedman test results showed a highly significant effect of the type of generation in the answers regarding the stimuli being or not generated with AI ($\chi^2(5)=51.59$, $p<.001$). As it is observable from the corresponding violin plot, participants were able to correctly detect which of the groups corresponded to the human-generated compositions. 

However, results from the pairwise Wilcoxon test (presented in Table \ref{tab:q7wilcoxon} of Appendix A) revealed no statistically significant differences amongst pairs of groups, except for the combinations of \textbf{progrand-proghum}, \textbf{progrand-rockhum} and \textbf{proghum-rockcp}, and comparisons between the AI-generated Rock groups (\textbf{rockrand} and \textbf{rockcp}) agaisnt the human-generated Rock group (\textbf{rockhum}). We highlight the answers for groups \textbf{progcp} and, surprisingly, \textbf{rockrand}, for which participants could not confidently tell if they were AI-generated or not (a median score of ``Neutral'').

The plot in Figure \ref{fig:isrep} displays the results to Q8, concerning the repetitiveness of the compositions. We report a highly significant effect of the type of generation towards this variable ($H(5)=79.20$, $p<.001$).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/chapter-progGP/is_repetitive_violin_plot.pdf}
    \caption{Violin plot concerning the answers to Q8, ``This composition is repetitive''. }
    \label{fig:isrep}
\end{figure}

Regarding the pairwise Wilcoxon test (displayed in Table \ref{tab:q8wilcoxon} of Appendix A), results did not show any conclusive outcomes, with some combinations presenting statistically significant differences between groups, whereas the same could not be said for other pairs. We highlight that the comparisons \textbf{progcp-proghum} and \textbf{progcp-rockhum} obtained similar median scores from participants (``Neutral'').

\subsection{Thematic Analysis}




==> Tables/turingtest.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c|c}
\hline
\textbf{Subset} & \textbf{CE loss} \\
\hline
\hline
Overall & 1.2509 \\
\hline
Progressive Metal & 1.3014 \\
\hline
Rock & 1.2005 \\
\hline
Cherry-picked & 1.5461 \\
\hline
Random & 1.2441 \\
\hline
Human & 6.7032 \\
\hline
progcp & 1.8546 \\
\hline
rockcp& 1.2375 \\
\hline
progrand& 0.7827 \\
\hline
rockrand & 1.7054 \\
\hline
proghum & 4.7532 \\
\hline
rockhum & 8.6532 \\
\hline
\hline
\end{tabular}
\end{center}
\caption{Average CE classification error for AI- vs. human-composed over different subsets of the test stimuli.}
\label{tab:turingtest}
\end{table}

